On the Expressive Power of Kernel Methods and the Efficiency of Kernel Learning by Association Schemes

We study the expressive power of kernel methods and the algorithmic feasibility of multiple kernel learning for a special rich class of kernels. Specifically, we define \emph{Euclidean kernels}, a diverse class that includes most, if not all, families of kernels studied in literature such as polynomial kernels and radial basis functions. We then describe the geometric and spectral structure of this family of kernels over the hypercube (and to some extent for any compact domain). Our structural results allow us to prove meaningful limitations on the expressive power of the class as well as derive several efficient algorithms for learning kernels over different domains.

==> content/conjunction-upper-bound.tex <==
%!TEX root=../arxiv_main.tex
\section{Proof of \thmref{thm:upper}}

We next discuss how margin assumption can improve guarantees when certain distribution assumptions are made. In particular we prove \thmref{thm:upper}. Again, for simplicity and due to similar arguments as in \secref{sec:hypercube} we assume that $\|\xx\|=s$ almost surely (having $\|\xx\|\le s$ will only lead to a linear dependency in $s$ which is negligible w.r.t $2^s$).

We also simplify by learning conjunctions with a fixed number of literals $\ell\le s$ (again, to learn all conjunctions, this will lead to a polynomial scale in $s$). The kernel of our choice to learn the problem is the kernel given by the base kernels suggested by the Johnson Scheme analysis. Namely we choose the $s$-th element in the $P$ basis introduced in \defref{def:pbasis}. Concretely we let $k_{\ell}$ be defined by
\[ k(\s{x}{i},\s{x}{j}) = {{s}\choose{\ell}}^{-1}\cdot {{\s{x}{i}\cdot \s{x}{j}}\choose{\ell}}.\]
To show that the kernel learns the class of conjunctions with $\ell$ literals in time $\mathrm{poly}(2^s,\frac{1}{\epsilon},\log 1/\delta)$ it would be enough to show that if $H$ is the associated Hilbert space then there is $\ww\in H$ such that $\|\ww\|\le 2^s$ and
\begin{align*}
\dotp{\ww}{\phi(\s{x}{i})} = c_{I}.
\end{align*}
We can then employ $L_1$ regression algorithm (or in fact any surrogate loss funciton) to learn the class. Indeed, given the conjunction $c_{I}$ let $\mathbf{c}$ be a vector such that $\mathbf{c}_i = 1$ for all $i\in I$ and $\mathbf{c}_i=0$ else. If we let $\ww={s\choose \ell}\phi(\mathbf{c})$ then one can verify that:
\begin{align*}
\dotp{\ww}{\phi(\xx)} = {{\mathbf{c}\cdot \xx}\choose{\ell}} = 
\begin{cases}
1 &  \sum_{i\in I} \s{x}{i} =\ell \\ 
0 & \mathrm{else}  
\end{cases} = c_{I}(\xx).
\end{align*}
The element $\phi(\mathbf{c})$ belongs to $H$ and we have that

\begin{align*}
\|{s\choose \ell} \phi(\mathbf{c})\|^2 = {s\choose \ell}^2{s\choose \ell}^{-1} {{\mathbf{c}\cdot \mathbf{c}}\choose{\ell}}= {s\choose \ell} = O(2^s).
\end{align*}

\paragraph{Comparison to other methods and algorithms} It is worth comparing the result to the standard approach of polynomial approximation. Standard methods to learn conjunctions rely on a Chebyshev's polynomial approximation of degree $O(\sqrt{n})$. Over sparse distribution like the one we are considering here, the approximation implies a polynomial with monomials of degree at most $s$. Namely, for every conjunction $c_I$ there exists a polynomial $p_{I}$ of degree $O(s)$ over $n$ variables such that for every $\xx$ with $\sum \s{x}{i}=s$ we have
\[|c_{I}(\xx) - p(\xx)| < \epsilon\]
This result implies an algorithm (through learning an $L_1$ regressor in monomial space) with complexity $O(n^s)= O(2^{s\log n})$ where here we obtain a learning rate of $O(2^s)$. 


